Realizing Learned Quadruped Locomotion Behaviors through Kinematic Motion Primitives

Humans and animals are believed to use a very minimal set of trajectories to perform a wide variety of tasks including walking. Our main objective in this paper is two fold 1) Obtain an effective tool to realize these basic motion patterns for quadrupedal walking, called the kinematic motion primitives (kMPs), via trajectories learned from deep reinforcement learning (D-RL) and 2) Realize a set of behaviors, namely trot, walk, gallop and bound from these kinematic motion primitives in our custom four legged robot, called the `Stoch'. D-RL is a data driven approach, which has been shown to be very effective for realizing all kinds of robust locomotion behaviors, both in simulation and in experiment. On the other hand, kMPs are known to capture the underlying structure of walking and yield a set of derived behaviors. We first generate walking gaits from D-RL, which uses policy gradient based approaches. We then analyze the resulting walking by using principal component analysis. We observe that the kMPs extracted from PCA followed a similar pattern irrespective of the type of gaits generated. Leveraging on this underlying structure, we then realize walking in Stoch by a straightforward reconstruction of joint trajectories from kMPs. This type of methodology improves the transferability of these gaits to real hardware, lowers the computational overhead on-board, and also avoids multiple training iterations by generating a set of derived behaviors from a single learned gait.

==> temp.tex <==
Section \ref{sec:results/HWexp} describes the results of the implementation of kMP in the hardware. Section \ref{subsubsec: data_compare} shows the comparison of the kMP between the trot gaits learned in robot simulation, implemented in hardware and extracted from horse. Horse kMP was extracted by digitizing the plots from \cite{moro2013horse}. The tables in this section report only the final results of the statistics applied. In section \ref{subsubsec: Gait_change}, we change gait from trot to pace and vice verse by just switching the elements of the weight matrix. In section \ref{subsubsec: Turning}, we generate turning motion by manipulating the weights of the weight matrix.
\subsubsection{Experimental setup}\label{subsubsec: Exp_setup}
The experiments on the hardware is conducted on flat terrain. the details of the test can be seen in these\textbf{VIDEO} videos.
All the tests were conducted at 2.5 Hz frequency.  
\subsubsection{Data comparison}\label{subsubsec: data_compare}


\begin{figure*}[h!]
\centering
\includegraphics[width=\linewidth]{kMP_trot_grd.pdf}
  \caption{kMP for trot}
  \label{fig:kMP_trot}
\end{figure*}


Some of the kMPs, as it can be seen, share some common features with other gaits. To observe if these gaits a have any common kMP we super impose one plot over. Following diagram  shows the superimposed plot.

While analyzing the data, we compared the extracted kMP with some of the kMP of animals found in the literature. A comparison with the horse kMP can be seen in the figure \ref{fig:kMP_BioVsRL}. 
\begin{figure}[h!]
\includegraphics[width=\linewidth]{kMP_HorseVsRL.pdf}
  \caption{Comparison between the horse kMP and the RL learned kMP in trot gait}
  \label{fig:kMP_BioVsRL}
\end{figure}

\begin{table}
\centering
\begin{tabular}{c||c|c|c|c||c|c}
 & 1st & 2nd & 3rd & 4th & Average & Weighted\\
\hline
RLT1-RLT2 & 0.99 & 0.93 & 0.82 & 0.78 & - & -\\
RLT1-HT & 0.951 & 0.979 & 0.936 & 0.656 & - & - \\
RLT2-HT & 0.97 & 0.99 & 0.77 & 0.55 & - & - 
\end{tabular}
\caption{Statistical analysis of similarity among kMPs extracted from Reinforcement learned trot(RLT1 and RLT2) and Horse trot kmp(HT) - cross-covariance}
\end{table}
\begin{table}[h!]
\centering
\begin{tabular}{c||c|c|c|c||c|c}
 & 1st & 2nd & 3rd & 4th & Average & Weighted\\
\hline
RLT1-RLT2 & 0 & -0.02 & -0.09 & -0.01 & - & -\\
RLT1-HT & -0.03 & 0 & 0 & 0.5 & - & - \\
RLT2-HT & 0 & 0.02 & -0.1 & -0.05 & - & -
\end{tabular}
\caption{Statistical analysis of similarity among kMPs extracted from Reinforcement learned trot(RLT1 and RLT2) and Horse trot kmp(HT) - Delay}
\end{table}
